Machine Unlearning in Learned Databases: An Experimental Analysis

Machine learning models based on neural networks (NNs) are enjoying ever-increasing attention in the DB community. However, an important issue has been largely overlooked, namely the challenge of dealing with the highly dynamic nature of DBs, where data updates are fundamental, highly-frequent operations. Although some recent research has addressed the issues of maintaining updated NN models in the presence of new data insertions, the effects of data deletions (a.k.a., "machine unlearning") remain a blind spot. With this work, for the first time to our knowledge, we pose and answer the following key questions: What is the effect of unlearning algorithms on NN-based DB models? How do these effects translate to effects on downstream DB tasks, such as selectivity estimation (SE), approximate query processing (AQP), data generation (DG), and upstream tasks like data classification (DC)? What metrics should we use to assess the impact and efficacy of unlearning algorithms in learned DBs? Is the problem of machine unlearning in DBs different from that of machine learning in DBs in the face of data insertions? Is the problem of machine unlearning for DBs different from unlearning in the ML literature? what are the overhead and efficiency of unlearning algorithms? What is the sensitivity of unlearning on batching delete operations? If we have a suitable unlearning algorithm, can we combine it with an algorithm handling data insertions en route to solving the general adaptability/updatability requirement in learned DBs in the face of both data inserts and deletes? We answer these questions using a comprehensive set of experiments, various unlearning algorithms, a variety of downstream DB tasks, and an upstream task (DC), each with different NNs, and using a variety of metrics on a variety of real datasets, making this also a first key step towards a benchmark for learned DB unlearning.

==> figures_tex/dbest_census_loss_histograms.tex <==
\begin{figure*}
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/loss_distributions/census_stale_losses.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/loss_distributions/census_retrain_losses.png}}
\end{minipage} % 
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/loss_distributions/census_finetune_losses.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/loss_distributions/census_sgda_losses.png}}
\end{minipage} \\%

\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/loss_distributions/census_NegGrad_losses.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/loss_distributions/census_NegGrad+_losses.png}}
\end{minipage}%

\vspace{-0.3cm}
\caption{Histogram of losses of census dataset for different methods, on DBEst++}
\label{fig:dbest_census_losses}
\vspace{-0.4cm}
\end{figure*}

==> figures_tex/dbest_census_selective.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/census_histograms_dbest/census_train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/census_histograms_dbest/census_retrain_selective_real.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/census_histograms_dbest/census_retrain_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/census_histograms_dbest/census_stale_selective_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/census_histograms_dbest/census_finetune_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/census_histograms_dbest/census_SCRUB_selective_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:g}\includegraphics[scale=.25]{figures/census_histograms_dbest/census_NegGrad+_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:h}\includegraphics[scale=.25]{figures/census_histograms_dbest/census_NegGrad_selective_synthetic.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{Histogram of column ``age'' for Census dataset where Native-Country=`` United States''. Here we have performed ``Selective'' deletion.}
\label{fig:dbest_census_selective}
\vspace{-0.1cm}
\end{figure}

==> figures_tex/dbest_dmv_full.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_retrain_full_real.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_retrain_full_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_stale_full_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_finetune_full_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_SCRUB_full_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:g}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_NegGrad+_full_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:h}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_NegGrad_full_synthetic.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{histogram of column 'max gross weight' for DMV dataset where body-type='PICK'. Here we have performed ``Full'' deletion. }
\label{fig:dbest_dmv_full}
\vspace{-0.1cm}
\end{figure}

==> figures_tex/dbest_dmv_selective.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_retrain_selective_real.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_retrain_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_stale_selective_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_finetune_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_SCRUB_selective_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:g}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_NegGrad+_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:h}\includegraphics[scale=.25]{figures/dmv_histograms_dbest/dmv_NegGrad_selective_synthetic.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{Histogram of column ``max gross weight'' for DMV dataset where body-type=``PICK''. Here we have performed ``Selective'' deletion. }
\label{fig:dbest_dmv_selective}
\vspace{-0.1cm}
\end{figure}

==> figures_tex/dbest_forest_full.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_retrain_full_real.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_retrain_full_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_stale_full_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_finetune_full_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_SCRUB_full_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:g}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_NegGrad+_full_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:h}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_NegGrad_full_synthetic.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{Histogram of column ``Elevation'' for forest dataset where Slope=``11''. Here we have performed ``Full'' deletion. }
\label{fig:dbest_forest_full}
\vspace{-0.1cm}
\end{figure}

==> figures_tex/dbest_forest_loss_histograms_full.tex <==
\begin{figure*}
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/loss_distributions/forest_stale_losses.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/loss_distributions/forest_retrain_losses.png}}
\end{minipage} % 
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/loss_distributions/forest_finetune_losses.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/loss_distributions/forest_sgda_losses.png}}
\end{minipage} \\%

\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/loss_distributions/forest_NegGrad_losses.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/loss_distributions/forest_NegGrad+_losses.png}}
\end{minipage}%

\vspace{-0.3cm}
\caption{Distribution of loss values for DBEst++ model for Forest dataset, after full deletion using different methods. In this experiment we first split the data into train and test partitions. We train the model using the train-set and delete a part of data from only the train-set. The plots then compare the distribution of losses for the train-set (without the deleted rows), the held-out test-set, and the delete-set.  }
\label{fig:dbest_forest_losses_full}
\vspace{-0.4cm}
\end{figure*}

==> figures_tex/dbest_forest_loss_histograms_selective.tex <==
\begin{figure*}
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/loss_distributions/forest_stale_losses_selective.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/loss_distributions/forest_retrain_losses_selective.png}}
\end{minipage} % 
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/loss_distributions/forest_finetune_losses_selective.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/loss_distributions/forest_SCRUB_losses_selective.png}}
\end{minipage} \\%

\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/loss_distributions/forest_NegGrad+_losses_selective.png}}
\end{minipage}%
\begin{minipage}{.24\textwidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/loss_distributions/forest_NegGrad_losses_selective.png}}
\end{minipage}%

\vspace{-0.3cm}
\caption{Distribution of loss values for DBEst++ model for Forest dataset, after selective deletion using different methods. In this experiment we first split the data into train and test partitions. We train the model using the train-set and delete a part of data from only the train-set. The plots then compare the distribution of losses for the train-set (without the deleted rows), the held-out test-set, and the delete-set.}
\label{fig:dbest_forest_losses_selective}
\vspace{-0.4cm}
\end{figure*}

==> figures_tex/dbest_forest_selective.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_retrain_selective_real.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_retrain_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_stale_selective_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_finetune_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_SCRUB_selective_synthetic.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:g}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_NegGrad+_selective_synthetic.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:h}\includegraphics[scale=.25]{figures/forest_histograms_dbest/forest_NegGrad_selective_synthetic.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{Histogram of column ``Elevation'' for forest dataset where Slope=``11''. Here we have performed ``Selective'' deletion. }
\label{fig:dbest_forest_selective}
\vspace{-0.1cm}
\end{figure}

==> figures_tex/tvae_census_full.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Retrain_real_full.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Retrain_synthetic_full.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Stale_synthetic_full.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Finetune_synthetic_full.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_NegGrad+_synthetic_full.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{Histogram of ``age'' for Census. DG/TVAE. ``Full'' deletion.}
\label{fig:tvawe_census_full}
\vspace{-0.1cm}
\end{figure}

==> figures_tex/tvae_census_selective.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Retrain_real_selective.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Retrain_synthetic_selective.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Stale_synthetic_selective.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_Finetune_synthetic_selective.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/census_histograms_tvae/census_NegGrad+_synthetic_selective.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{Histogram of column ``age'' for Census dataset for TVAE when performing ``Selective'' deletion.}
\label{fig:tvawe_census_selective}
\vspace{-0.1cm}
\end{figure}

==> figures_tex/tvae_forest_full.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Retrain_real_full.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Retrain_synthetic_full.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Stale_synthetic_full.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Finetune_synthetic_full.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_NegGrad+_synthetic_full.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{Histogram of column ``Elevation'' for Forest dataset for TVAE when performing ``Full'' deletion.}
\label{fig:tvawe_forest_full}
\vspace{-0.1cm}
\end{figure}

==> figures_tex/tvae_forest_selective.tex <==
\begin{figure}[!ht]
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:a}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Train_real.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:b}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Retrain_real_selective.png}}
\end{minipage} % 
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:c}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Retrain_synthetic_selective.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:d}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Stale_synthetic_selective.png}}
\end{minipage} \\%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:e}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_Finetune_synthetic_selective.png}}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\subfloat[]{\label{main:f}\includegraphics[scale=.25]{figures/forest_histograms_tvae/forest_NegGrad+_synthetic_selective.png}}
\end{minipage}
\vspace{-0.1cm}
\caption{Histogram of column ``Elevation'' for Forest dataset for TVAE when performing ``Full'' deletion.}
\label{fig:tvawe_forest_full}
\vspace{-0.1cm}
\end{figure}

==> tables/combined_tables_9_10.tex <==
\begin{table}
\parbox{.45\textwidth}{
\centering
    \begin{tabular}{c | c | c c }
\toprule
dataset&model&Full Deletion&Selective Deletion \\
\midrule
\multirow{6}{*}{Census}
%&Original&12.97±0.91&12.97±0.91\\
%\cmidrule{2-4}
&Retrain&16.87±1.08&14.32±1.07\\
&Stale&16.20±0.86&13.81±0.99\\
&Fine-tune&10.23±0.71&9.48±0.79\\
&NegGrad+&10.42±0.70&9.19±0.79\\
&NegGrad&97.62±26.17&107.35±43.48\\
&SCRUB&11.71±0.74&10.93±0.87\\

\midrule

\multirow{6}{*}{Forest}
%&Original&19.92±1.97&19.92±1.97\\
%\cmidrule{2-4}
&Retrain&24.96±4.44&21.66±1.99\\
&Stale&23.78±4.61&20.78±1.71\\
&Fine-tune&21.48±3.67&18.34±1.64\\
%&Fine-tune&22.46±4.49&18.73±1.69\\
&NegGrad+&22.43±4.61&19.38±2.05\\
&NegGrad&74.23±18.83&76.81±17.15\\
&SCRUB&23.12±4.78&19.94±1.86\\

\midrule
\multirow{6}{*}{DMV}
%&Original&9.54±1.66&9.54±1.66 \\
%\cmidrule{2-4}
&Retrain&7.37±0.58&8.68±0.61\\
&Stale&13.63±0.61&11.95±1.00\\
&Fine-tune&5.13±0.56&5.77±0.66\\
%&Fine-tune&6.03±0.54&5.77±0.66\\
&NegGrad+&5.34±0.56&9.06±0.70\\
&NegGrad&2892.63±3283.17&40.90±2.63\\
&SCRUB&18.67±1.87&10.25±0.91\\

\midrule
    \end{tabular}
\caption{The full and selective deletion results for SE/Naru-NeuroCard. The numbers in the table are average relative-error and 95 \% confidence interval for remain queries-QR (full deletion) and queries covering remain and deleted data (selective deletion).}
}
\hfill
\parbox{.45\textwidth}{
\centering
\begin{tabular}{c | c | c c | c c }
    \toprule
         \multirow{2}{*}{dataset}&\multirow{2}{*}{model}&\multicolumn{2}{c|}{Full Deletion}&\multicolumn{2}{c}{Selective Deletion}  \\
         &&retain synth&delete synth&retain synth&deleted synth \\
         \midrule
         
\multirow{4}{*}{Census}
%&Original&73.81±0.41&60.36±0.73&-&-&73.81±0.41&60.36±0.73&-&-\\
%\cmidrule{2-10}
&Retrain&61.13±0.84&62.84±3.99&61.33±0.93&69.79±0.99\\
&Stale&61.27±0.19&69.33±0.71&60.77±0.95&70.10±0.33\\
&Fine-tune&60.11±1.18&68.84±0.49&61.32±1.18&70.18±0.21\\
&NegGrad+&60.41±0.83&69.09±1.01&61.35±0.65&69.80±1.07\\

\midrule

\multirow{4}{*}{Forest}
%&Original&81.86±0.44&46.63±1.35&-&-&81.86±0.44&46.63±1.35&-&-\\
%\cmidrule{2-10}
&Retrain&41.46±1.00&16.39±0.87&44.57±0.77&21.55±2.66\\
&Stale&46.94±0.80&32.31±1.83&46.15±0.46&32.49±1.68\\
&Fine-tune&48.39±1.49&28.85±2.04&48.89±0.73&34.65±1.07\\
&NegGrad+&49.95±0.78&31.16±1.16&46.32±1.01&33.74±1.13\\
\midrule

\multirow{4}{*}{DMV}
%&Original&45.88±0.61&40.88±0.39&-&-&45.88±0.61&40.88±0.39&-&-\\
%\cmidrule{2-10}
&Retrain&41.69±0.72&36.19±3.76&41.02±0.40&43.64±1.62\\\
&Stale&41.12±0.51&36.99±4.47&41.12±0.48&35.70±5.44\\
&Fine-tune&41.34±0.51&36.08±1.19&40.39±0.29&37.59±5.05\\
&NegGrad+&40.72±0.56&37.40±4.12&41.22±0.72&52.21±6.96\\
\midrule
    \end{tabular}
\caption{Full and selective deletion results for DG/TVAE. `retain synth' refers to the f1-score of the xgboost classifier when trained with synthetic data and evaluated on the held-out test-set. `delete synth' refers to the f1-score of the xgboost classifier when trained with the synth data and evaluate on the deleted rows.}
}
\end{table}

==> tables/dbest_census_full.tex <==
\begin{comment}
\begin{table*}[]
  \centering
    \caption{DBEst-census-Full}
    \label{tab:mdn_census_full}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c c c c c | c c c c c c | c c}
\toprule
\multirow{2}{*}{model}&\multicolumn{6}{c|}{queries on the retain rows}&\multicolumn{6}{c|}{queries on the deleted rows}&\multicolumn{2}{c}{likelihood}\\
&mean-cnt&median-cnt&99th-cnt&mean-sum&median-sum&99th-sum&mean-cnt&median-cnt&99th-cnt&mean-sum&median-sum&99th-sum&deleted&retained \\
\midrule
original & 24.49 & 1.26 & 895.38 & 662.65 & 65.81 & 25848.87 &-&-&-&-&-&-&-&- \\
\midrule
SCRUBS & 13.52 & 1.90 & 265.95 & 1252.58 & 95.63 & 35535.15 & 3.98 & 3.17 & 9.25 & 219.59 & 122.59 & 806.19 & 0.13&0.88 \\
NegGrad & 130.76 & 10.10 & 5258.70 & 6475.32 & 472.46 & 259299.61 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00&0.18 \\
NegGrad+ & 16.16 & 2.41 & 212.59 & 1129.09 & 110.96 & 33200.60 & 0.12 & 0.00 & 1.26 & 20.39 & 0.42 & 120.38 & 0.03&0.98 \\
Fine-tune & 10.65 & 1.58 & 274.03 & 926.22 & 70.86 & 37610.55 & 2.18 & 1.40 & 6.17 & 120.49 & 63.55 & 556.64 & 0.07 & 0.96 \\
Stale & 39.64 & 2.74 & 999.52 & 2626.32 & 112.05 & 79994.00 & 16.06 & 15.06 & 32.97 & 1469.38 & 531.64 & 6698.73 &0.96&0.70 \\
Retrain & 9.51 & 1.23 & 164.34 & 992.30 & 65.88 & 33412.29 & 0.39 & 0.22 & 1.77 & 51.74 & 12.80 & 469.67 & 0.03 & 0.99 \\
\midrule
    \end{tabular}}
\end{table*}
\end{comment}

\begin{table*}[]
  \centering
    \caption{DBEst-census-Full}
    \label{tab:mdn_census_full}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c c c c c | c c c c c c | c c}
\toprule
\multirow{2}{*}{model}&\multicolumn{6}{c|}{queries on the retain rows}&\multicolumn{6}{c|}{queries on the deleted rows}&\multicolumn{2}{c}{likelihood}\\
&mean-cnt&median-cnt&95th-cnt&mean-sum&median-sum&95th-sum&mean-cnt&median-cnt&95th-cnt&mean-sum&median-sum&95th-sum&retained&deleted \\
\midrule
Original & 14.75 & 6.60 & 54.18 & 14.94 & 7.79 & 54.34 &-&-&-&-&-&-&-&-\\
\midrule
Retrain & 18.16 & 9.46 & 59.53 & 18.03 & 8.77 & 58.57 & 0.35 & 0.31 & 0.73 & 483.68 & 16.26 & 666.80 & 1.00 & 0.03 \\
Stale & 32.05 & 24.94 & 69.18 & 37.16 & 25.99 & 83.13 & 26.22 & 20.33 & 62.18 & 30410.04 & 481.07 & 299146.18 & 0.71 & 0.97 \\
Fine-tune & 19.44 & 12.73 & 56.55 & 19.91 & 10.37 & 67.67 & 3.94 & 1.77 & 12.07 & 1791.61 & 72.72 & 14811.48 & 0.96 & 0.08 \\
NegGrad+ & 34.26 & 17.75 & 94.23 & 29.87 & 17.45 & 101.84 & 0.21 & 0.00 & 0.62 & 601.70 & 0.96 & 646.38 & 0.98 & 0.03 \\
NegGrad & 177.99 & 81.23 & 727.74 & 161.54 & 80.14 & 606.63 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.17 & 0.00 \\
SCRUB & 26.91 & 15.50 & 87.59 & 25.63 & 14.18 & 86.96 & 4.45 & 4.01 & 9.36 & 4149.24 & 99.70 & 31436.97 & 0.89 & 0.14 \\
\midrule

    \end{tabular}}
\end{table*}

==> tables/dbest_census_ratio_deleted.tex <==
\begin{table}
\small
    \centering
        \caption{The ratio of absolute-errors when deleting in one-go over sequential deletion. The numbers show the results for DBEst++ model with Census dataset when evaluating delete queries. For each method, the top line is when deleting in one-go, and the second line is when deleting sequentially.}
    \label{tab:census_ratio_numbers}
      \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c c | c c c}
    \toprule
         \multirow{2}{*}{method}&\multicolumn{3}{c|}{count queries}&\multicolumn{3}{c}{sum queries}\\
         &average&median&95th&average&median&95th  \\
        \midrule
Retrain & 0.09 & 0.00 & 0.12 & 2.29 & 0.13 & 4.07\\
Retrain & 0.12 & 0.01 & 0.17 & 3.90 & 0.28 & 4.66\\
\midrule
Stale & 26.62 & 1.97 & 22.61 & 824.70 & 63.76 & 763.31\\
Stale & 26.62 & 1.97 & 22.61 & 824.70 & 63.76 & 763.31\\
\midrule
Fine-tune & 0.83 & 0.22 & 1.62 & 24.69 & 7.60 & 54.54\\
Fine-tune & 0.84 & 0.19 & 1.29 & 24.12 & 6.19 & 43.18\\
\midrule
NegGrad+ & 0.27 & 0.03 & 1.79 & 11.34 & 0.99 & 49.18\\
NegGrad+ & 0.26 & 0.00 & 1.60 & 12.13 & 0.01 & 46.39\\
\midrule
NegGrad & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
NegGrad & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00\\
\midrule
SCRUB & 1.94 & 0.51 & 3.31 & 57.48 & 16.88 & 105.81\\
SCRUB & 1.80 & 0.53 & 3.51 & 55.89 & 17.54 & 115.85\\
\midrule
    \end{tabular}}

\end{table}

==> tables/dbest_census_selective.tex <==
\begin{comment}
\begin{table*}
  \centering
    \caption{DBEst-census-Selective}
    \label{tab:mdn_census_selective}
    \begin{tabular}{c | c c c c c c | c c}
\toprule
\multirow{2}{*}{model}&\multirow{2}{*}{mean-cnt}&\multirow{2}{*}{median-cnt}&\multirow{2}{*}{99th-cnt}&\multirow{2}{*}{mean-sum}&\multirow{2}{*}{median-sum}&\multirow{2}{*}{99th-sum}&\multicolumn{2}{c}{likelihood} \\
&&&&&&&deleted&retained\\
\midrule
original & 24.49 & 1.26 & 895.38 & 662.65 & 65.81 & 25848.87 & - & -\\
\midrule
SCRUBS & 14.01 & 1.28 & 505.62 & 738.33 & 64.95 & 22484.26 & 0.62 & 0.76 \\
NegGrad & 323.57 & 12.59 & 12943.22 & 12321.55 & 542.00 & 475598.47 & 0.00 & 0.15 \\
NegGrad+ & 16.62 & 1.31 & 520.02 & 783.30 & 58.82 & 22138.69 & 0.47 & 0.78 \\
Fine-tune & 13.99 & 1.19 & 660.85 & 732.89 & 63.98 & 27109.41 & 0.62 & 0.77 \\
Stale & 31.12 & 1.56 & 1358.42 & 1475.89 & 79.24 & 48109.95 & 0.96 & 0.75 \\
Retrain & 17.85 & 1.19 & 784.89 & 760.40 & 58.29 & 23309.98 & 0.60 & 0.77 \\
\midrule
    \end{tabular}
\end{table*}
\end{comment}

\begin{table*}
  \centering
    \caption{DBEst-census-Selective}
    \label{tab:mdn_census_selective}
    \begin{tabular}{c | c c c c c c | c c}
\toprule
\multirow{2}{*}{model}&\multirow{2}{*}{mean-cnt}&\multirow{2}{*}{median-cnt}&\multirow{2}{*}{95th-cnt}&\multirow{2}{*}{mean-sum}&\multirow{2}{*}{median-sum}&\multirow{2}{*}{95th-sum}&\multicolumn{2}{c}{likelihood} \\
&&&&&&&retained&deleted\\
\midrule
Original & 14.75 & 6.60 & 54.18 & 14.94 & 7.79 & 54.34 &-&-\\
\midrule
Retrain & 14.12 & 7.07 & 51.86 & 17.35 & 7.97 & 65.40 & 0.78 & 0.60 \\
Stale & 17.90 & 11.48 & 56.15 & 21.02 & 13.58 & 64.95 & 0.75 & 0.97 \\
Fine-tune & 14.98 & 7.20 & 54.77 & 17.69 & 8.77 & 60.59 & 0.77 & 0.62 \\
NegGrad+ & 14.93 & 7.51 & 49.57 & 17.92 & 8.06 & 62.65 & 0.79 & 0.47 \\
NegGrad & 145.12 & 81.87 & 447.18 & 208.67 & 90.19 & 923.37 & 0.15 & 0.00 \\
SCRUB & 16.23 & 8.62 & 53.21 & 18.96 & 9.39 & 62.36 & 0.76 & 0.76 \\
\midrule
    \end{tabular}
\end{table*}

==> tables/dbest_dmv_full.tex <==
\begin{comment}
\begin{table*}
  \centering
    \caption{DBEst-DMV-Full}
    \label{tab:mdn_dmv_full}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c c c c c | c c c c c c | c c }
\toprule
\multirow{2}{*}{model}&\multicolumn{6}{c|}{queries on the retain rows}&\multicolumn{6}{c|}{queries on the deleted rows}&\multicolumn{2}{c}{likelihood}\\
&mean-cnt&median-cnt&99th-cnt&mean-sum&median-sum&99th-sum&mean-cnt&median-cnt&99th-cnt&mean-sum&median-sum&99th-sum&deleted&retained \\
\midrule
original & 99.25 & 0.00 & 1552.35 & 2248579.81 & 0.04 & 56791756.18 &-&-&-&-&-&-&-&- \\
\midrule
SCRUBS & 149.46 & 0.00 & 3887.41 & 9678683.36 & 9.34 & 162048973.05 & 48.41 & 0.33 & 476.98 & 15720.44 & 2443.70 & 118139.54 & 40.45 & 29.15  \\
NegGrad & 1360.25 & 0.00 & 25290.78 & 142980211.01 & 0.00 & 3397507986.56 & 0.04 & 0.00 & 0.67 & 11.90 & 0.00 & 185.26 & 0.00 & 0.39 \\
NegGrad+ & 43.27 & 0.00 & 770.11 & 5131503.90 & 0.76 & 26273157.52 & 0.23 & 0.03 & 2.26 & 4231.02 & 822.47 & 20824.17 & 0.37 & 49.87 \\
Fine-tune & 47.38 & 0.00 & 1300.84 & 4867923.11 & 0.36 & 66122950.46 & 18.44 & 0.04 & 202.33 & 6251.36 & 1018.63 & 36141.47 & 47.21 & 38.04 \\
Stale & 37.16 & 0.00 & 702.66 & 4105660.12 & 0.22 & 58692607.96 & 60.85 & 0.04 & 662.39 & 8781.61 & 1574.16 & 41929.10 & 87.78 & 34.33 \\
Retrain & 86.18 & 0.00 & 2827.75 & 5434276.93 & 0.36 & 66066176.52 & 26.52 & 0.03 & 279.35 & 4016.24 & 704.64 & 22467.59 & 44.46 & 39.43\\
\midrule
    \end{tabular}}
\end{table*}
\end{comment}

\begin{table*}
  \centering
    \caption{DBEst-DMV-Full}
    \label{tab:mdn_dmv_full}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c c c c c | c c c c c c | c c }
\toprule
\multirow{2}{*}{model}&\multicolumn{6}{c|}{queries on the retain rows}&\multicolumn{6}{c|}{queries on the deleted rows}&\multicolumn{2}{c}{likelihood}\\
&mean-cnt&median-cnt&95th-cnt&mean-sum&median-sum&95th-sum&mean-cnt&median-cnt&95th-cnt&mean-sum&median-sum&95th-sum&retained&deleted \\
\midrule
Original & 52.83 & 27.39 & 112.25 & 73.25 & 23.38 & 157.26 &-&-&-&-&-&-&-&-  \\
\midrule
Retrain & 75.73 & 34.41 & 246.04 & 310.98 & 47.35 & 347.28 & 263.50 & 0.49 & 2468.40 & 1710612.06 & 104896.17 & 11573505.32 & 68.43 & 5.69 \\
Stale & 62.68 & 34.87 & 174.08 & 109.19 & 37.77 & 190.67 & 3983.97 & 0.83 & 38076.59 & 13664630.82 & 399942.68 & 121292144.90 & 40.35 & 38.27 \\
Fine-tune & 72.84 & 34.96 & 145.18 & 92.40 & 36.49 & 356.11 & 491.09 & 0.83 & 4107.20 & 3873828.82 & 268297.89 & 28718864.73 & 48.28 & 7.36 \\
NegGrad+ & 66.32 & 28.08 & 264.76 & 108.51 & 37.22 & 273.29 & 24.80 & 0.36 & 57.44 & 737346.71 & 57254.54 & 4223017.16 & 47.37 & 0.15 \\
NegGrad+ & 48.99 & 30.52 & 136.81 & 83.19 & 33.46 & 287.51 & 30.62 & 0.44 & 101.72 & 1189284.73 & 157101.44 & 5627024.08 & 53.92 & 0.89 \\
NegGrad & 463.65 & 91.20 & 2715.49 & 1561.14 & 93.22 & 2237.82 & 0.39 & 0.00 & 2.23 & 1079.97 & 0.01 & 1092.89 & 0.13 & 0.00 \\
SCRUB & 279.67 & 63.07 & 2056.57 & 902.64 & 68.09 & 2816.88 & 8308.78 & 1.00 & 35958.06 & 60797602.66 & 198353.94 & 167273158.06 & 24.46 & 37.09 \\
\midrule
    \end{tabular}}
\end{table*}

==> tables/dbest_dmv_selective.tex <==
\begin{comment}
\begin{table*}
  \centering
    \caption{DBEst-DMV-Selective}
    \label{tab:mdn_dmv_selective}
    \begin{tabular}{c | c c c c c c | c c }
    \toprule
\multirow{2}{*}{model}&\multirow{2}{*}{mean-cnt}&\multirow{2}{*}{median-cnt}&\multirow{2}{*}{99th-cnt}&\multirow{2}{*}{mean-sum}&\multirow{2}{*}{median-sum}&\multirow{2}{*}{99th-sum}&\multicolumn{2}{c}{likelihood} \\
&&&&&&&deleted&retained\\
\midrule
original & 99.25 & 0.00 & 1552.35 & 2248579.81 & 0.04 & 56791756.18 & - & - \\
\midrule
SCRUBS & 149.31 & 0.00 & 1609.81 & 7209011.77 & 3.57 & 256408971.21 & 88.74 & 35.36\\
NegGrad & 3786.18 & 0.00 & 121201.47 & 89258211.03 & 0.00 & 1380027602.33 & 0.00 & 0.37 \\
NegGrad+ & 50.16 & 0.00 & 1399.82 & 5826081.59 & 1.63 & 91267938.21 & 66.43 & 37.51\\
Fine-tune & 93.44 & 0.00 & 1665.85 & 4886481.89 & 1.56 & 63192695.17 & 73.07 & 48.49\\
Stale & 71.24 & 0.00 & 1340.19 & 3862097.04 & 0.55 & 84681851.66 & 87.81 & 37.68\\
Retrain & 143.11 & 0.00 & 3527.36 & 11231878.46 & 0.10 & 150530220.46 & 71.76 & 38.63\\
\midrule
    \end{tabular}
\end{table*}
\end{comment}

\begin{table*}
  \centering
    \caption{DBEst-DMV-Selective}
    \label{tab:mdn_dmv_selective}
    \begin{tabular}{c | c c c c c c | c c }
    \toprule
\multirow{2}{*}{model}&\multirow{2}{*}{mean-cnt}&\multirow{2}{*}{median-cnt}&\multirow{2}{*}{95th-cnt}&\multirow{2}{*}{mean-sum}&\multirow{2}{*}{median-sum}&\multirow{2}{*}{95th-sum}&\multicolumn{2}{c}{likelihood} \\
&&&&&&&retained&deleted\\
\midrule
Original & 52.83 & 27.39 & 112.25 & 73.25 & 23.38 & 157.26 &-&-  \\
\midrule
Retrain & 73.00 & 33.17 & 284.40 & 95.41 & 37.70 & 150.75 & 67.32 & 153.95 \\
Stale & 54.80 & 34.48 & 118.30 & 62.50 & 29.95 & 257.79 & 40.12 & 38.27 \\
Fine-tune & 58.36 & 39.11 & 160.07 & 57.34 & 25.66 & 134.30 & 39.84 & 30.23 \\
NegGrad+ & 208.14 & 28.00 & 113.37 & 36.25 & 21.93 & 97.00 & 40.08 & 23.14 \\
NegGrad+ & 161.16 & 32.07 & 235.80 & 46.59 & 23.23 & 118.56 & 41.01 & 27.57 \\
NegGrad & 99.92 & 100.00 & 100.00 & 100.38 & 100.00 & 100.00 & 0.00 & 0.00 \\
SCRUB & 189.94 & 39.58 & 405.45 & 181.53 & 40.39 & 345.95 & 37.83 & 38.64 \\
\midrule

    \end{tabular}
\end{table*}





==> tables/dbest_forest_full.tex <==
\begin{comment}
\begin{table*}
  \centering
    \caption{DBEst-forest-Full}
    \label{tab:mdn_forest_full}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c c c c c | c c c c c c | c c }
\toprule
\multirow{2}{*}{model}&\multicolumn{6}{c|}{queries on the retain rows}&\multicolumn{6}{c|}{queries on the deleted rows}&\multicolumn{2}{c}{likelihood}\\
&mean-cnt&median-cnt&99th-cnt&mean-sum&median-sum&99th-sum&mean-cnt&median-cnt&99th-cnt&mean-sum&median-sum&99th-sum&deleted&retained \\
\midrule
original & 30.40 & 8.22 & 235.77 & 78725.63 & 21202.60 & 684808.26 &-&-&-&-&-&-&-&- \\
\midrule
SCRUBS & 29.52 & 5.60 & 215.53 & 86811.60 & 19319.32 & 696484.98 & 8.82 & 0.48 & 45.67 & 30082.58 & 5196.65 & 154354.81 & 0.00 & 1.31 \\
NegGrad & 610.21 & 56.09 & 5738.45 & 1707455.71 & 216021.52 & 13769656.43 & 1.39 & 0.67 & 5.11 & 3343.12 & 653.66 & 30483.42 & 0.00 & 1.45 \\
NegGrad+ & 52.70 & 7.76 & 409.16 & 158580.48 & 19299.58 & 1508968.55 & 0.12 & 0.03 & 0.87 & 3054.21 & 151.43 & 27097.93 & 0.00 & 1.31 \\
Fine-tune & 29.11 & 5.62 & 239.58 & 98308.09 & 16853.77 & 860461.78 & 6.68 & 0.44 & 29.38 & 26668.27 & 3887.57 & 110494.56 & 0.00 & 1.31 \\
Stale & 212.07 & 26.39 & 1348.05 & 596231.24 & 81516.88 & 3877161.86 & 412.40 & 44.41 & 1491.05 & 905468.93 & 189568.19 & 3484321.99 & 0.34 & 1.23 \\
Retrain & 25.73 & 4.42 & 223.23 & 73171.52 & 14259.71 & 634668.50 & 6.68 & 0.21 & 35.69 & 21944.95 & 2666.27 & 82603.56 & 0.00 & 1.31 \\
\midrule
    \end{tabular}}
\end{table*}
\end{comment}

\begin{table*}
  \centering
    \caption{DBEst-forest-Full}
    \label{tab:mdn_forest_full}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c c c c c | c c c c c c | c c }
\toprule
\multirow{2}{*}{model}&\multicolumn{6}{c|}{queries on the retain rows}&\multicolumn{6}{c|}{queries on the deleted rows}&\multicolumn{2}{c}{likelihood}\\
&mean-cnt&median-cnt&95th-cnt&mean-sum&median-sum&95th-sum&mean-cnt&median-cnt&95th-cnt&mean-sum&median-sum&95th-sum&retained&deleted \\
\midrule
Original & 9.84 & 2.54 & 52.19 & 11.02 & 3.13 & 44.55 &-&-&-&-&-&-&-&- \\
\midrule
Retrain & 10.85 & 2.00 & 50.20 & 10.78 & 3.22 & 49.78 & 10.81 & 6.80 & 35.81 & 28655.32 & 20281.26 & 83688.80 & 1.32 & 0.00 \\
Stale & 22.26 & 16.22 & 57.36 & 22.09 & 18.03 & 57.43 & 562.51 & 172.72 & 1441.59 & 1418393.03 & 1002536.48 & 3398392.76 & 1.23 & 0.34 \\
Fine-tune & 12.20 & 2.44 & 53.24 & 11.36 & 3.48 & 55.65 & 10.53 & 5.55 & 34.85 & 28914.40 & 18128.45 & 79991.75 & 1.31 & 0.00 \\
NegGrad+ & 13.99 & 4.91 & 54.45 & 13.83 & 5.20 & 56.48 & 0.00 & 0.00 & 0.01 & 14061.41 & 4.09 & 16550.34 & 1.31 & 0.00 \\
NegGrad+ & 14.08 & 4.94 & 58.19 & 13.46 & 5.17 & 54.90 & 1.11 & 0.03 & 10.24 & 18230.07 & 175.22 & 68875.53 & 1.31 & 0.00 \\
NegGrad & 120.19 & 24.01 & 343.10 & 77.02 & 25.57 & 226.67 & 5.29 & 1.48 & 37.68 & 2793.75 & 1501.58 & 9738.98 & 1.43 & 0.00 \\
SCRUB & 11.82 & 2.68 & 57.25 & 11.76 & 3.32 & 53.51 & 12.47 & 5.50 & 36.63 & 36531.91 & 29002.51 & 92407.93 & 1.31 & 0.00 \\
\midrule
    \end{tabular}}
\end{table*}

==> tables/dbest_forest_ratio_deleted.tex <==
\begin{table}
\small
    \centering
        \caption{The ratio of absolute-errors when deleting in one-go over sequential deletion. The numbers show the results for DBEst++ model with Forest dataset when evaluating delete queries. For each method, the top line is when deleting in one-go, and the second line is when deleting sequentially.}
    \label{tab:forest_ratio_numbers}
      \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c c | c c c}
    \toprule
         \multirow{2}{*}{method}&\multicolumn{3}{c|}{count queries}&\multicolumn{3}{c}{sum queries}\\
         &average&median&95th&average&median&95th  \\
        \midrule
Retrain & 0.00 & 0.00 & 0.02 & 0.69 & 0.05 & 2.69\\
Retrain & 0.00 & 0.00 & 0.02 & 0.74 & 0.05 & 3.70\\
\midrule
Stale & 4.23 & 1.55 & 14.20 & 9148.42 & 2864.52 & 34294.81\\
Stale & 4.23 & 1.55 & 14.20 & 9148.42 & 2864.52 & 34294.81\\
\midrule
Fine-tune & 0.01 & 0.00 & 0.04 & 14.68 & 1.45 & 44.05\\
Fine-tune & 0.01 & 0.00 & 0.05 & 58.26 & 2.57 & 308.43\\
\midrule
NegGrad+ & 0.00 & 0.00 & 0.00 & 1.75 & 0.00 & 0.00\\
NegGrad+ & 0.00 & 0.00 & 0.00 & 0.67 & 0.00 & 1.08\\
\midrule
NegGrad & 0.00 & 0.00 & 0.00 & 0.63 & 0.00 & 0.08\\
NegGrad & 0.00 & 0.00 & 0.00 & 22.58 & 0.00 & 10.50\\
\midrule
SCRUB & 0.05 & 0.01 & 0.23 & 72.93 & 12.70 & 297.54\\
SCRUB & 0.05 & 0.01 & 0.22 & 70.78 & 11.11 & 310.94\\
\midrule
    \end{tabular}}

\end{table}


==> tables/dbest_forest_selective.tex <==
\begin{comment}
\begin{table*}
  \centering
    \caption{DBEst-forest-Selective}
    \label{tab:mdn_forest_selective}
    \begin{tabular}{c | c c c c c c | c c }
    \toprule
\multirow{2}{*}{model}&\multirow{2}{*}{mean-cnt}&\multirow{2}{*}{median-cnt}&\multirow{2}{*}{99th-cnt}&\multirow{2}{*}{mean-sum}&\multirow{2}{*}{median-sum}&\multirow{2}{*}{99th-sum}&\multicolumn{2}{c}{likelihood} \\
&&&&&&&deleted&retained\\
\midrule
original & 30.40 & 8.22 & 235.77 & 78725.63 & 21202.60 & 684808.26 & - & - \\
\midrule
sgda & 24.77 & 5.07 & 231.55 & 59048.07 & 10384.18 & 519334.41 & 0.20 & 1.22 \\
NegGrad & 652.17 & 78.34 & 6226.28 & 1677665.19 & 87771.29 & 15550390.46 & 0.00 & 1.39 \\
NegGrad+ & 69.48 & 13.66 & 431.73 & 190373.26 & 24816.57 & 1188478.09 & 0.09 & 1.24 \\
Fine-tune & 21.37 & 5.28 & 205.62 & 57489.19 & 9599.31 & 523614.56 & 0.20 & 1.23 \\
Stale & 102.14 & 19.95 & 722.27 & 289658.87 & 42554.57 & 1843937.67 & 0.34 & 1.20 \\
Retrain & 21.43 & 5.48 & 215.79 & 63666.79 & 11128.31 & 538589.96 & 0.19 & 1.23 \\
\midrule
    \end{tabular}
\end{table*}
\end{comment}


\begin{table*}
  \centering
    \caption{DBEst-forest-Selective}
    \label{tab:mdn_forest_selective}
    \begin{tabular}{c | c c c c c c | c c }
    \toprule
\multirow{2}{*}{model}&\multirow{2}{*}{mean-cnt}&\multirow{2}{*}{median-cnt}&\multirow{2}{*}{95th-cnt}&\multirow{2}{*}{mean-sum}&\multirow{2}{*}{median-sum}&\multirow{2}{*}{95th-sum}&\multicolumn{2}{c}{likelihood} \\
&&&&&&&retained&deleted\\
\midrule
Original & 9.84 & 2.54 & 52.19 & 11.02 & 3.13 & 44.55 & - & - \\
\midrule
Retrain & 9.58 & 2.18 & 45.16 & 9.62 & 2.87 & 43.13 & 1.23 & 0.20 \\
Stale & 22.48 & 9.35 & 98.16 & 20.54 & 9.50 & 72.42 & 1.20 & 0.34 \\
Fine-tune & 9.51 & 2.16 & 44.12 & 9.77 & 2.52 & 43.16 & 1.23 & 0.20 \\
NegGrad+ & 26.42 & 11.81 & 100.00 & 27.06 & 13.85 & 100.00 & 1.26 & 0.00 \\
NegGrad+ & 16.55 & 7.04 & 63.64 & 17.20 & 7.22 & 59.42 & 1.25 & 0.10 \\
NegGrad & 72.99 & 28.84 & 128.00 & 69.27 & 35.68 & 171.55 & 1.37 & 0.00 \\
SCRUB & 10.11 & 2.36 & 43.77 & 9.92 & 2.90 & 43.26 & 1.23 & 0.20 \\

\midrule
    \end{tabular}
\end{table*}






==> tables/naru_census_full.tex <==
\begin{comment}
\begin{table}[]
  \centering
    \caption{Naru-census-Full}
    \label{tab:naru_census_full}

    \begin{tabular}{c | c c c }
\toprule
model&mean-cnt&median-cnt&99th-cnt \\
\midrule
original & 50.92 & 4.00 & 702.30 \\
\midrule
SCRUBS & 69.73 & 4.00 & 914.22 \\
NegGrad & 508.08 & 17.00 & 8332.35 \\
NegGrad+ & 45.57 & 3.50 & 711.84 \\
Fine-tune & 31.02 & 3.00 & 423.02 \\
Stale & 112.94 & 5.00 & 1432.00 \\
Retrain & 43.11 & 3.00 & 757.08 \\
\midrule
    \end{tabular}
\end{table}
\end{comment}


\begin{table}[]
  \centering
    \caption{Naru-census-Full}
    \label{tab:naru_census_full}

    \begin{tabular}{c | c c c }
\toprule
model&mean-cnt&median-cnt&95th-cnt \\
\midrule
original & 12.81 & 5.83 & 50.02 \\
\midrule
SCRUB&16.97&12.83&50.00 \\
%SCRUB&20.67&16.42&50.16 \\
NegGrad&93.65&97.17&99.99 \\
%NegGrad+&26.20&19.88&75.00 \\
%NegGrad+&18.15&12.51&50.00 \\
NegGrad+&14.57&9.05&47.21 \\
Fine-tune&14.83&8.84&45.76 \\
Fine-tune&12.29&6.08&50.00 \\
Stale&23.13&23.28&54.15 \\
Retrain&14.82&8.47&50.00 \\
\midrule
    \end{tabular}
\end{table}

==> tables/naru_census_selective.tex <==
\begin{comment}
\begin{table}[]
  \centering
    \caption{Naru-census-Selective}
    \label{tab:naru_census_selective}

    \begin{tabular}{c | c c c }
\toprule
model&mean-cnt&median-cnt&99th-cnt \\
\midrule
original & 50.92 & 4.00 & 702.30 \\
\midrule
SCRUBS & 41.62 & 4.00 & 549.68 \\
NegGrad & 642.88 & 26.00 & 9805.45 \\
NegGrad+ & 22.16 & 3.00 & 305.37 \\
Fine-tune & 25.53 & 3.00 & 343.17 \\
Stale & 62.89 & 5.00 & 868.98 \\
Retrain & 66.75 & 4.00 & 1048.13 \\
\midrule
    \end{tabular}
\end{table}

\end{comment}
\begin{table}[]
  \centering
    \caption{Naru-census-Selective}
    \label{tab:naru_census_selective}

    \begin{tabular}{c | c c c }
\toprule
model&mean-cnt&median-cnt&95th-cnt \\
\midrule
original & 12.81 & 5.83 & 50.02 \\
\midrule
SCRUB&11.63&6.20&40.80 \\
%SCRUB&14.74780376&9.061692705&50 \\
NegGrad&97.642&98.24&99.99 \\
%NegGrad+&11.36389176&6.127353197&41.93283315 \\
%NegGrad+&10.28223401&4.973254707&40 \\
NegGrad+&9.19&3.84&33.33 \\
Fine-tune&9.81&4.27&37.17 \\
%Finetune&11.12694318&5.626156093&50 \\
Stale&15.80&10.27&50.00 \\
Retrain&16.56&9.60&53.39 \\
\midrule
    \end{tabular}
\end{table}

==> tables/naru_dmv_full.tex <==
\begin{comment}
\begin{table}
  \centering
    \caption{Naru-dmv-Full}
    \label{tab:naru_dmv_full}

    \begin{tabular}{c | c c c}
\toprule
model&mean-cnt&median-cnt&99th-cnt \\
\midrule
original & 1640.99 & 181.50 & 16645.05 \\
\midrule
SCRUBS & 4642.27 & 264.00 & 59488.07 \\
NegGrad & 8415.38 & 525.50 & 85242.84 \\
NegGrad+ & 4505.32 & 283.00 & 49613.02 \\
Fine-tune & 2629.11 & 187.50 & 27704.04 \\
Stale & 6080.35 & 345.00 & 69292.43 \\
Retrain & 1770.51 & 202.00 & 18299.58 \\
\midrule
    \end{tabular}
\end{table}
\end{comment}

\begin{table}
  \centering
    \caption{Naru-dmv-Full}
    \label{tab:naru_dmv_full}

    \begin{tabular}{c | c c c}
\toprule
model&mean-cnt&median-cnt&95th-cnt \\
\midrule
Original&7.48&3.89&25.72 \\
\midrule
SCRUB&14.45&9.99&40.98 \\
NegGrad&27.08&18.74&80.50 \\
NegGrad+&15.03&10.77&44.09 \\
Fine-tune&8.63&6.05&26.37 \\
Stale&18.13&12.79&53.93 \\
Retrain&10.48&6.30&40.00 \\
\midrule
    \end{tabular}
\end{table}

==> tables/naru_dmv_selective.tex <==
\begin{comment}
\begin{table}
  \centering
    \caption{Naru-dmv-Selective}
    \label{tab:naru_dmv_selective}
    \begin{tabular}{c | c c c}
\toprule
model&mean-cnt&median-cnt&99th-cnt \\
\midrule
original & 1640.99 & 181.50 & 16645.05 \\
\midrule
SCRUBS & 2864.04 & 319.00 & 35091.83 \\
NegGrad & 9801.45 & 834.50 & 104492.36 \\
NegGrad+ & 3551.02 & 288.00 & 33933.83 \\
Fine-tune & 826.92 & 87.00 & 8891.71 \\
Stale & 3710.17 & 298.50 & 44818.66 \\
Retrain & 1385.33 & 166.00 & 12241.21 \\
\midrule
    \end{tabular}
\end{table}
\end{comment}


\begin{table}
  \centering
    \caption{Naru-dmv-Selective}
    \label{tab:naru_dmv_selective}
    \begin{tabular}{c | c c c}
\toprule
model&mean-cnt&median-cnt&95th-cnt \\
\midrule
Original&7.48&3.89&25.72 \\
\midrule
SCRUB&10.18&5.90&33.87 \\
NegGrad&30.35&21.18&83.61 \\
NegGrad+&12.98&8.39&37.54 \\
Fine-tune&5.49&2.08&22.94 \\
Stale&12.26&7.95&37.50 \\
Retrain&6.90&3.29&23.76 \\
\midrule
    \end{tabular}
\end{table}

==> tables/naru_forest_full.tex <==
\begin{comment}
\begin{table}
  \centering
    \caption{Naru-forest-Full}
    \label{tab:naru_forest_full}
    \begin{tabular}{c | c c c |}
\toprule
model&mean-cnt&median-cnt&99th-cnt \\
\midrule
train & 312.97 & 2.00 & 5263.20 \\
\midrule
SCRUBS & 379.61 & 2.00 & 8388.91 \\
NegGrad & 2687.12 & 5.00 & 63143.99 \\
NegGrad+ & 321.51 & 2.00 & 8649.82 \\
Fine-tune & 230.29 & 2.00 & 4522.54 \\
Stale & 508.56 & 3.00 & 10802.26 \\
Retrain & 286.94 & 2.00 & 7130.64 \\
\midrule
    \end{tabular}
\end{table}
\end{comment}

\begin{table}
  \centering
    \caption{Naru-forest-Full}
    \label{tab:naru_forest_full}
    \begin{tabular}{c | c c c }
\toprule
model&mean-cnt&median-cnt&95th-cnt \\
\midrule
Original & 19.54 & 5.20 & 73.42 \\
\midrule
SCRUB&24.57&5.57&70.38 \\
NegGrad&56.80&33.14&154.82 \\
NegGrad+&22.20&6.02&66.67 \\
%Finetune&22.82&5.80&66.67 \\
Fine-tune&21.17&5.03&66.67 \\
Stale&27.66&7.84&67.74 \\
Retrain&34.72&6.19&71.90 \\
\midrule
    \end{tabular}
\end{table}

==> tables/naru_forest_selective.tex <==
\begin{comment}
\begin{table}
  \centering
    \caption{Naru-forest-Selective}
    \label{tab:naru_forest_selective}

    \begin{tabular}{c | c c c |}
\toprule
model&mean-cnt&median-cnt&99th-cnt \\
\midrule
train & 312.97 & 2.00 & 5263.20 \\
\midrule
scrubs & 255.44 & 2.00 & 4957.89 \\
NegGrad & 2774.16 & 5.00 & 67179.75 \\
NegGrad+ & 244.25 & 2.00 & 5770.11 \\
Fine-tune & 217.32 & 2.00 & 4767.21 \\
Stale & 335.04 & 2.50 & 6019.58 \\
Retrain & 259.58 & 2.00 & 4783.31 \\
\midrule
    \end{tabular}
\end{table}
\end{comment}


\begin{table}
  \centering
    \caption{Naru-forest-Selective}
    \label{tab:naru_forest_selective}

    \begin{tabular}{c | c c c }
\toprule
model&mean-cnt&median-cnt&95th-cnt \\
\midrule
Original & 19.54 & 5.20 & 73.42 \\
\midrule
SCRUB&23.94&4.94&70.27 \\
NegGrad&67.88&31.98&153.46 \\
NegGrad+&28.39&4.11&71.44 \\
%Finetune&25.44&3.78&71.56 \\
Fine-tune&21.46&4.27&66.83 \\
Stale&27.36&6.01&75.00 \\
Retrain&33.92&5.61&75.00 \\
\midrule
    \end{tabular}
\end{table}

==> tables/tvae_census_selective.tex <==
\begin{table}[]
  \centering
    \caption{TVAE-census-Selective}
    \label{tab:tvae_census_selective}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c | c c | c c | c c }
\toprule
\multirow{2}{*}{model}&\multicolumn{2}{c}{retain real}&\multicolumn{2}{c}{retain synth}& \multicolumn{2}{c}{deleted real}&\multicolumn{2}{c}{deleted synth}\\
&avg&std&avg&std&avg&std&avg&std \\
\midrule
Original &81.51&0.00&75.95&0.00&-&-&-&- \\
\midrule
Retrain&80.81&0.00&75.87&0.00&79.74&0.00&71.59&0.00 \\
Stale&80.81&0.00&76.81&0.00&79.74&0.00&68.86&0.00 \\
Fine-tune&80.81&0.00&75.01&0.00&79.74&0.00&66.85&0.00 \\
NegGrad+&80.81&0.00&75.67&0.00&79.74&0.00&66.24&0.00 \\
%NegGrad&81.45&0.00&19.15&0.00&79.74&0.00&21.09&0.00 \\

\midrule
    \end{tabular}}
\end{table}

==> tables/tvae_dmv_full.tex <==
\begin{table}
  \centering
    \caption{tvae-DMV-Full}
    \label{tab:tvae_dmv_full}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c | c c | c c | c c }
\toprule
\multirow{2}{*}{model}&\multicolumn{2}{c}{real}&\multicolumn{2}{c}{synth}& \multicolumn{2}{c}{deleted}&\multicolumn{2}{c}{deleted synth}\\
&avg&std&avg&std&avg&std&avg&std \\
\midrule
Original&44.62&0.00&39.81&0.00&-&-&-&- \\
\midrule
Retrain&46.27&0.00&41.07&0.00&41.35&0.00&44.00&0.00 \\
Stale&46.27&0.00&39.80&0.00&41.35&0.00&34.36&0.00 \\
Fine-tune&46.27&0.00&41.04&0.00&41.35&0.00&34.36&0.00 \\
NegGrad+&46.27&0.00&40.72&0.00&41.35&0.00&34.36&0.00 \\

\midrule
    \end{tabular}}
\end{table}

==> tables/tvae_dmv_selective.tex <==
\begin{table}
  \centering
    \caption{tvae-DMV-Selective}
    \label{tab:tvae_dmv_selective}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c | c c | c c | c c }
\toprule
\multirow{2}{*}{model}&\multicolumn{2}{c}{real}&\multicolumn{2}{c}{synth}& \multicolumn{2}{c}{deleted}&\multicolumn{2}{c}{deleted synth}\\
&avg&std&avg&std&avg&std&avg&std \\
\midrule
Original&44.62&0.00&39.81&0.00&-&-&-&- \\
\midrule
Retrain&46.86&0.00&40.57&0.00&45.29&0.00&45.29&0.00 \\
Stale&46.86&0.00&40.69&0.00&42.95&0.00&33.11&0.00 \\
Fine-tune&46.86&0.00&40.58&0.00&33.08&0.00&33.08&0.00 \\
NegGrad+&46.86&0.00&40.82&0.00&43.57&0.00&41.75&0.00 \\

\midrule
    \end{tabular}}
\end{table}


==> tables/tvae_forest_full.tex <==
\begin{table}
  \centering
    \caption{tvae-forest-Full}
    \label{tab:tvae_forest_full}
      \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c | c c | c c | c c}
\toprule
\multirow{2}{*}{model}&\multicolumn{2}{c}{real}&\multicolumn{2}{c}{synth}& \multicolumn{2}{c}{deleted}&\multicolumn{2}{c}{deleted synth}\\
&avg&std&avg&std&avg&std&avg&std \\
\midrule
Original&81.89&0.00&44.14&0.00&-&-&-&- \\
\midrule
Retrain&69.34&0.00&33.55&0.00&32.58&0.00&12.74&0.00 \\
Stale&69.34&0.00&33.86&0.00&32.58&0.00&25.85&0.00 \\
Fine-tune&69.34&0.00&34.60&0.00&32.58&0.00&18.15&0.00 \\
NegGrad+&69.34&0.00&33.72&0.00&32.58&0.00&20.34&0.00 \\

\midrule
    \end{tabular}}
\end{table}

==> tables/tvae_forest_selective.tex <==
\begin{table}
  \centering
    \caption{tvae-forest-Selective}
    \label{tab:tvae_forest_selective}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c | c c | c c | c c | c c}
\toprule
\multirow{2}{*}{model}&\multicolumn{2}{c}{real}&\multicolumn{2}{c}{synth}& \multicolumn{2}{c}{deleted}&\multicolumn{2}{c}{deleted synth}\\
&avg&std&avg&std&avg&std&avg&std \\
\midrule
Original&81.89&0.00&44.14&0.00&-&-&-&- \\
\midrule
Retrain&80.79&0.00&40.08&0.00&80.54&0.00&25.45&0.00 \\
Stale&80.79&0.00&42.72&0.00&80.54&0.00&26.29&0.00 \\
Fine-tune&80.79&0.00&41.95&0.00&80.54&0.00&24.43&0.00 \\
NegGrad+&80.79&0.00&40.91&0.00&80.54&0.00&25.16&0.00 \\

\midrule
    \end{tabular}}
\end{table}
